Articulation Upper Bounds for Language Models

Language captures only a subset of the perceptions, intuitions and intents that form meaning between speakers. What, then, are the limits of language? We take steps towards measuring this in LLMs as follows: for a set of concepts, we measure how well each concept can be transmitted between two LLMs as their capabilities scale. This requires novel measurement tools: (1) optimal messages: we introduce a prompt optimization algorithm that beats existing algorithms by up to 14% on benchmarks and accurately estimates prompt upper bounds. (2) A transmission measure: the sender is asked to label text; the receiver then tries to recover the sender's prompt, and recovery is measured; we find this correlates strongly with human label error. With these measures, we use observational scaling laws to study how transmissibility of a concept, conveyed with optimal messages, increases as transmitter and receiver capacity grows: does it asymptote below or above a threshold? Measuring 1.2k concepts in eight domains, we find concepts that (a) can be fully articulated; these concepts usually depend on local patterns, e.g. "joke ends with surprise"; (b) might be articulated by future, stronger models; these rely on whole-text structural patterns, e.g. "story's worldbuilding coherence"; (c) concepts that face articulability limits; these concepts' meaning, we find, is tied to identity and social-group awareness, e.g. "comic voice". Interesting, these same concepts are not all challenging for humans: humans have moderate-to-high levels of agreement in 76% of concepts that LLMs struggle with; articulation limits, we find, are executor relative. Finally, we characterize the nature of improvement in each case: while recoverable concepts can be articulated through definitions and explanations, irrecoverable concepts cannot be transmitted, even with examples, and might require novel learning mechanisms.

==> figs/gen_change_types_simple.tex <==
\fill[green!25, draw=green!50!black, line width=0.5pt] (0,2.34) rectangle (9.20,2.96);
\node[font=\tiny] at (4.60,2.65) {definition 51\% $+$ explanation 49\%};
\node[tlab, anchor=east, align=right] at (-0.18,2.65) {tacit decompression\\(name$\to$def$\to$expl)\\ ($n{=}200$)};
\node[font=\tiny, anchor=west, text=green!40!black] at (9.32,2.65) {100\%};
\fill[green!25, draw=green!50!black, line width=0.5pt] (0,1.17) rectangle (0.07,1.79);
\fill[blue!12, draw=blue!50!black, line width=0.5pt] (0.07,1.17) rectangle (9.20,1.79);
\node[font=\tiny] at (4.64,1.48) {score anchors \& format 77\% $\cdot$ input hygiene 12\% $\cdot$ edge cases 10\%};
\node[tlab, anchor=east, align=right] at (-0.18,1.48) {GEPA rounds\\ ($n{=}203$)};
\node[font=\tiny, anchor=west, text=green!40!black] at (9.32,1.48) {0.8\%};
\fill[green!25, draw=green!50!black, line width=0.5pt] (0,0.00) rectangle (0.25,0.62);
\fill[blue!12, draw=blue!50!black, line width=0.5pt] (0.25,0.00) rectangle (9.20,0.62);
\node[font=\tiny] at (4.72,0.31) {checking steps 47\% $\cdot$ score anchors 18\% $\cdot$ edge cases 11\%};
\node[tlab, anchor=east, align=right] at (-0.18,0.31) {$M_\omega$ unit additions\\ ($n{=}360$)};
\node[font=\tiny, anchor=west, text=green!40!black] at (9.32,0.31) {3\%};
\fill[green!25, draw=green!50!black] (0,3.56) rectangle (0.22,3.70);
\node[font=\tiny, anchor=west] at (0.27,3.63) {concept content (definition, explanation)};
\fill[blue!12, draw=blue!50!black] (4.4,3.56) rectangle (4.62,3.70);
\node[font=\tiny, anchor=west] at (4.67,3.63) {measurement content (anchors, checks, \ldots)};
\node[font=\tiny, anchor=south, text=green!40!black] at (9.65,3.23) {\% concept};



==> figs/gen_osl_domains.tex <==
\draw[-{Stealth[length=1.6mm]}] (-0.25,0) -- (-0.25,2.90);
\node[tlab, rotate=90] at (-1.1,1.30) {share of domain's metrics};
\draw (-0.31,0.00) -- (-0.19,0.00); \node[tlab, anchor=east] at (-0.34,0.00) {0\%};
\draw (-0.31,0.65) -- (-0.19,0.65); \node[tlab, anchor=east] at (-0.34,0.65) {25\%};
\draw (-0.31,1.30) -- (-0.19,1.30); \node[tlab, anchor=east] at (-0.34,1.30) {50\%};
\draw (-0.31,1.95) -- (-0.19,1.95); \node[tlab, anchor=east] at (-0.34,1.95) {75\%};
\draw (-0.31,2.60) -- (-0.19,2.60); \node[tlab, anchor=east] at (-0.34,2.60) {100\%};
\fill[red!22, draw=red!65!black, line width=0.5pt] (0.920,0.000) rectangle (0.000,2.038);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (0.460,1.019) {78};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (0.920,2.038) rectangle (0.000,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (0.460,2.319) {22};
\node[tlab, align=center, anchor=north] at (0.460,-0.08) {press\\releases\\($n{=}199$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (2.260,0.000) rectangle (1.340,2.229);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (1.800,1.114) {86};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (2.260,2.229) rectangle (1.340,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (1.800,2.414) {14};
\node[tlab, align=center, anchor=north] at (1.800,-0.08) {patents\\($n{=}7$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (3.600,0.000) rectangle (2.680,2.285);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (3.140,1.142) {88};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (3.600,2.285) rectangle (2.680,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (3.140,2.442) {12};
\node[tlab, align=center, anchor=north] at (3.140,-0.08) {notice\\and comment\\($n{=}66$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (4.940,0.000) rectangle (4.020,2.088);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (4.480,1.044) {80};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (4.940,2.088) rectangle (4.020,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (4.480,2.344) {20};
\node[tlab, align=center, anchor=north] at (4.480,-0.08) {math\\($n{=}137$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (6.280,0.000) rectangle (5.360,1.962);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (5.820,0.981) {75};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (6.280,1.962) rectangle (5.360,2.586);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (5.820,2.274) {24};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (6.280,2.586) rectangle (5.360,2.600);
\node[tlab, align=center, anchor=north] at (5.820,-0.08) {creative\\writing\\($n{=}367$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (7.620,0.000) rectangle (6.700,1.812);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (7.160,0.906) {70};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (7.620,1.812) rectangle (6.700,2.344);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (7.160,2.078) {20};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (7.620,2.344) rectangle (6.700,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=orange!80!black!25!black] at (7.160,2.472) {10};
\node[tlab, align=center, anchor=north] at (7.160,-0.08) {news\\homepages\\($n{=}132$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (8.960,0.000) rectangle (8.040,1.919);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (8.500,0.960) {74};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (8.960,1.919) rectangle (8.040,2.321);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (8.500,2.120) {15};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (8.960,2.321) rectangle (8.040,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=orange!80!black!25!black] at (8.500,2.461) {11};
\node[tlab, align=center, anchor=north] at (8.500,-0.08) {peer\\review\\($n{=}84$)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (10.300,0.000) rectangle (9.380,1.150);
\node[font=\fontsize{4.5}{5}\selectfont, text=red!65!black!25!black] at (9.840,0.575) {44};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (10.300,1.150) rectangle (9.380,2.217);
\node[font=\fontsize{4.5}{5}\selectfont, text=blue!60!black!25!black] at (9.840,1.683) {41};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (10.300,2.217) rectangle (9.380,2.600);
\node[font=\fontsize{4.5}{5}\selectfont, text=orange!80!black!25!black] at (9.840,2.408) {15};
\node[tlab, align=center, anchor=north] at (9.840,-0.08) {humor\\($n{=}278$)};
\fill[red!22, draw=red!65!black] (0.30,3.00) rectangle (0.54,3.15);
\node[font=\tiny, anchor=west] at (0.60,3.07) {rising};
\fill[blue!22, draw=blue!60!black] (3.90,3.00) rectangle (4.14,3.15);
\node[font=\tiny, anchor=west] at (4.20,3.07) {reaches its ceiling};
\fill[orange!30, draw=orange!80!black] (7.50,3.00) rectangle (7.74,3.15);
\node[font=\tiny, anchor=west] at (7.80,3.07) {bounded};



==> figs/gen_osl_types.tex <==
\node[font=\scriptsize\bfseries, anchor=west] at (0,3.13) {where do the criterion's truth conditions live?};
\fill[blue!18, draw=blue!60!black] (0.10,2.68) rectangle (0.36,2.84);
\node[font=\tiny, anchor=west] at (0.42,2.76) {in-text};
\fill[orange!30, draw=orange!80!black] (3.10,2.68) rectangle (3.36,2.84);
\node[font=\tiny, anchor=west] at (3.42,2.76) {at the interface};
\fill[red!25, draw=red!70!black] (6.10,2.68) rectangle (6.36,2.84);
\node[font=\tiny, anchor=west] at (6.42,2.76) {beyond the text};
\fill[blue!18, draw=blue!60!black, line width=0.5pt] (0.00,1.72) rectangle (6.27,2.24);
\node[font=\fontsize{5}{5}\selectfont, text=blue!60!black!30!black] at (3.13,1.98) {73\%};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (6.27,1.72) rectangle (7.61,2.24);
\node[font=\fontsize{5}{5}\selectfont, text=orange!80!black!30!black] at (6.94,1.98) {16\%};
\fill[red!25, draw=red!70!black, line width=0.5pt] (7.61,1.72) rectangle (8.60,2.24);
\node[font=\fontsize{5}{5}\selectfont, text=red!70!black!30!black] at (8.10,1.98) {12\%};
\node[font=\scriptsize\itshape, anchor=east] at (-0.12,1.98) {rising ($n{=}884$)};
\node[font=\tiny\itshape, anchor=west, text=black!55] at (8.72,1.98) {mean idx 0.39};
\fill[blue!18, draw=blue!60!black, line width=0.5pt] (0.00,0.86) rectangle (6.05,1.38);
\node[font=\fontsize{5}{5}\selectfont, text=blue!60!black!30!black] at (3.03,1.12) {70\%};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (6.05,0.86) rectangle (7.53,1.38);
\node[font=\fontsize{5}{5}\selectfont, text=orange!80!black!30!black] at (6.79,1.12) {17\%};
\fill[red!25, draw=red!70!black, line width=0.5pt] (7.53,0.86) rectangle (8.60,1.38);
\node[font=\fontsize{5}{5}\selectfont, text=red!70!black!30!black] at (8.06,1.12) {12\%};
\node[font=\scriptsize\itshape, anchor=east] at (-0.12,1.12) {reaches ($n{=}321$)};
\node[font=\tiny\itshape, anchor=west, text=black!55] at (8.72,1.12) {mean idx 0.42};
\fill[blue!18, draw=blue!60!black, line width=0.5pt] (0.00,0.00) rectangle (4.63,0.52);
\node[font=\fontsize{5}{5}\selectfont, text=blue!60!black!30!black] at (2.32,0.26) {54\%};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (4.63,0.00) rectangle (5.82,0.52);
\node[font=\fontsize{5}{5}\selectfont, text=orange!80!black!30!black] at (5.23,0.26) {14\%};
\fill[red!25, draw=red!70!black, line width=0.5pt] (5.82,0.00) rectangle (8.60,0.52);
\node[font=\fontsize{5}{5}\selectfont, text=red!70!black!30!black] at (7.21,0.26) {32\%};
\node[font=\scriptsize\itshape, anchor=east] at (-0.12,0.26) {bounded ($n{=}65$)};
\node[font=\tiny\itshape, anchor=west, text=black!55] at (8.72,0.26) {mean idx 0.78};



==> figs/gen_osl_types12.tex <==
\draw[-{Stealth[length=1.6mm]}] (-0.25,0) -- (-0.25,3.20);
\node[tlab, rotate=90] at (-0.85,1.45) {share of regime's metrics (\%)};
\draw (-0.31,0.00) -- (-0.19,0.00); \node[tlab, anchor=east] at (-0.34,0.00) {0};
\draw (-0.31,0.58) -- (-0.19,0.58); \node[tlab, anchor=east] at (-0.34,0.58) {10};
\draw[black!12] (-0.19,0.58) -- (15.60,0.58);
\draw (-0.31,1.16) -- (-0.19,1.16); \node[tlab, anchor=east] at (-0.34,1.16) {20};
\draw[black!12] (-0.19,1.16) -- (15.60,1.16);
\draw (-0.31,1.74) -- (-0.19,1.74); \node[tlab, anchor=east] at (-0.34,1.74) {30};
\draw[black!12] (-0.19,1.74) -- (15.60,1.74);
\draw (-0.31,2.32) -- (-0.19,2.32); \node[tlab, anchor=east] at (-0.34,2.32) {40};
\draw[black!12] (-0.19,2.32) -- (15.60,2.32);
\draw (-0.31,2.90) -- (-0.19,2.90); \node[tlab, anchor=east] at (-0.34,2.90) {50};
\draw[black!12] (-0.19,2.90) -- (15.60,2.90);
\draw (-0.25,0) -- (15.60,0);
\fill[red!22, draw=red!65!black, line width=0.5pt] (0.10,0) rectangle (0.44,0.256);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (0.27,0.264) {4};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (0.47,0) rectangle (0.81,0.379);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (0.64,0.387) {7};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (0.83,0) rectangle (1.17,0.178);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (1.00,0.186) {3};
\node[tlab, align=center, anchor=north] at (0.65,-0.08) {surface\\checks};
\fill[red!22, draw=red!65!black, line width=0.5pt] (1.40,0) rectangle (1.74,0.971);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (1.57,0.979) {17};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (1.77,0) rectangle (2.10,1.988);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (1.94,1.996) {34};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (2.13,0) rectangle (2.47,0.803);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (2.30,0.811) {14};
\node[tlab, align=center, anchor=north] at (1.95,-0.08) {local patterns\\(punchline, endings)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (2.70,0) rectangle (3.04,1.607);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (2.87,1.615) {28};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (3.07,0) rectangle (3.41,1.084);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (3.24,1.092) {19};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (3.43,0) rectangle (3.77,1.338);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (3.60,1.346) {23};
\node[tlab, align=center, anchor=north] at (3.25,-0.08) {extended\\structure};
\fill[red!22, draw=red!65!black, line width=0.5pt] (4.00,0) rectangle (4.34,0.551);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (4.17,0.559) {10};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (4.37,0) rectangle (4.71,0.434);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (4.54,0.442) {7};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (4.73,0) rectangle (5.07,0.446);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (4.90,0.454) {8};
\node[tlab, align=center, anchor=north] at (4.55,-0.08) {verification\\\& sourcing};
\fill[red!22, draw=red!65!black, line width=0.5pt] (5.30,0) rectangle (5.64,0.518);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (5.47,0.526) {9};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (5.67,0) rectangle (6.00,0.307);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (5.83,0.315) {5};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (6.03,0) rectangle (6.37,0.089);
\node[tlab, align=center, anchor=north] at (5.85,-0.08) {logical\\rigor};
\fill[red!22, draw=red!65!black, line width=0.5pt] (6.60,0) rectangle (6.94,0.223);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (6.77,0.231) {4};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (6.96,0) rectangle (7.30,0.181);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (7.13,0.189) {3};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (7.33,0) rectangle (7.67,0.357);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (7.50,0.365) {6};
\node[tlab, align=center, anchor=north] at (7.15,-0.08) {originality};
\fill[red!22, draw=red!65!black, line width=0.5pt] (7.90,0) rectangle (8.24,0.374);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (8.07,0.382) {6};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (8.27,0) rectangle (8.61,0.217);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (8.44,0.225) {4};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (8.63,0) rectangle (8.97,0.089);
\node[tlab, align=center, anchor=north] at (8.45,-0.08) {ethics \&\\harm};
\fill[red!22, draw=red!65!black, line width=0.5pt] (9.20,0) rectangle (9.54,0.420);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (9.37,0.428) {7};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (9.56,0) rectangle (9.90,0.307);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (9.73,0.315) {5};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (9.93,0) rectangle (10.27,0.268);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (10.10,0.276) {5};
\node[tlab, align=center, anchor=north] at (9.75,-0.08) {audience\\fit};
\fill[red!22, draw=red!65!black, line width=0.5pt] (10.50,0) rectangle (10.84,0.112);
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (10.87,0) rectangle (11.21,0.361);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (11.04,0.369) {6};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (11.23,0) rectangle (11.57,0.535);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (11.40,0.543) {9};
\node[tlab, align=center, anchor=north] at (11.05,-0.08) {community imit.\\\& stance};
\fill[red!22, draw=red!65!black, line width=0.5pt] (11.80,0) rectangle (12.14,0.164);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (11.97,0.172) {3};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (12.17,0) rectangle (12.51,0.108);
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (12.53,0) rectangle (12.87,0.803);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (12.70,0.811) {14};
\node[tlab, align=center, anchor=north] at (12.35,-0.08) {creator identity\\\& persona};
\fill[red!22, draw=red!65!black, line width=0.5pt] (13.10,0) rectangle (13.44,0.321);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (13.27,0.329) {6};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (13.46,0) rectangle (13.80,0.163);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (13.63,0.171) {3};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (13.83,0) rectangle (14.17,0.268);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (14.00,0.276) {5};
\node[tlab, align=center, anchor=north] at (13.65,-0.08) {ecosystem\\artifacts};
\fill[red!22, draw=red!65!black, line width=0.5pt] (14.40,0) rectangle (14.74,0.282);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=red!65!black] at (14.57,0.290) {5};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (14.77,0) rectangle (15.11,0.271);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=blue!60!black] at (14.94,0.279) {5};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (15.13,0) rectangle (15.47,0.625);
\node[font=\fontsize{4}{4.5}\selectfont, anchor=south, text=orange!80!black] at (15.30,0.633) {11};
\node[tlab, align=center, anchor=north] at (14.95,-0.08) {real-world\\reception};
\fill[red!22, draw=red!65!black] (0.60,3.30) rectangle (0.86,3.46);
\node[font=\scriptsize, anchor=west] at (0.92,3.38) {rising ($n{=}884$)};
\fill[blue!22, draw=blue!60!black] (5.60,3.30) rectangle (5.86,3.46);
\node[font=\scriptsize, anchor=west] at (5.92,3.38) {reaches its ceiling ($n{=}321$)};
\fill[orange!30, draw=orange!80!black] (10.60,3.30) rectangle (10.86,3.46);
\node[font=\scriptsize, anchor=west] at (10.92,3.38) {bounded below 1 ($n{=}65$)};



==> figs/gen_osl_types6.tex <==
\draw[-{Stealth[length=1.6mm]}] (-0.25,0) -- (-0.25,2.80);
\node[tlab, rotate=90] at (-0.85,1.25) {share of regime (\%)};
\draw (-0.31,0.00) -- (-0.19,0.00); \node[tlab, anchor=east] at (-0.34,0.00) {0};
\draw (-0.31,0.42) -- (-0.19,0.42); \node[tlab, anchor=east] at (-0.34,0.42) {10};
\draw[black!12] (-0.19,0.42) -- (12.30,0.42);
\draw (-0.31,0.83) -- (-0.19,0.83); \node[tlab, anchor=east] at (-0.34,0.83) {20};
\draw[black!12] (-0.19,0.83) -- (12.30,0.83);
\draw (-0.31,1.25) -- (-0.19,1.25); \node[tlab, anchor=east] at (-0.34,1.25) {30};
\draw[black!12] (-0.19,1.25) -- (12.30,1.25);
\draw (-0.31,1.67) -- (-0.19,1.67); \node[tlab, anchor=east] at (-0.34,1.67) {40};
\draw[black!12] (-0.19,1.67) -- (12.30,1.67);
\draw (-0.31,2.08) -- (-0.19,2.08); \node[tlab, anchor=east] at (-0.34,2.08) {50};
\draw[black!12] (-0.19,2.08) -- (12.30,2.08);
\draw (-0.31,2.50) -- (-0.19,2.50); \node[tlab, anchor=east] at (-0.34,2.50) {60};
\draw[black!12] (-0.19,2.50) -- (12.30,2.50);
\draw (-0.25,0) -- (12.30,0);
\fill[red!22, draw=red!65!black, line width=0.5pt] (0.12,0) rectangle (0.52,0.698);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=red!65!black] at (0.32,0.706) {17};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (0.55,0) rectangle (0.95,1.428);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=blue!60!black] at (0.75,1.436) {34};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (0.98,0) rectangle (1.38,0.577);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=orange!80!black] at (1.18,0.585) {14};
\node[tlab, align=center, anchor=north] at (0.75,-0.08) {Local patterns\\within document};
\fill[red!22, draw=red!65!black, line width=0.5pt] (2.17,0) rectangle (2.57,1.155); 
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=red!65!black] at (2.37,1.163) {28};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (2.60,0) rectangle (3.00,0.779);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=blue!60!black] at (2.80,0.787) {19};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (3.03,0) rectangle (3.43,0.962);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=orange!80!black] at (3.23,0.970) {23};
\node[tlab, align=center, anchor=north] at (2.80,-0.08) {Whole-text\\structural patterns};
\fill[red!22, draw=red!65!black, line width=0.5pt] (4.22,0) rectangle (4.62,1.221);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=red!65!black] at (4.42,1.229) {29};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (4.65,0) rectangle (5.05,0.961);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=blue!60!black] at (4.85,0.969) {23};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (5.08,0) rectangle (5.48,0.577);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=orange!80!black] at (5.28,0.585) {14};
\node[tlab, align=center, anchor=north] at (4.85,-0.08) {Verifiable\\features};
\fill[red!22, draw=red!65!black, line width=0.5pt] (6.27,0) rectangle (6.67,0.462);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=red!65!black] at (6.47,0.470) {11};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (6.70,0) rectangle (7.10,0.350);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=blue!60!black] at (6.90,0.358) {8};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (7.13,0) rectangle (7.53,0.449);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=orange!80!black] at (7.33,0.457) {11};
\node[tlab, align=center, anchor=north] at (6.90,-0.08) {Originality \&\\Audience fit};
\fill[red!22, draw=red!65!black, line width=0.5pt] (8.32,0) rectangle (8.72,0.198);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=red!65!black] at (8.52,0.206) {5};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (8.75,0) rectangle (9.15,0.337);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=blue!60!black] at (8.95,0.345) {8};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (9.18,0) rectangle (9.58,0.962);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=orange!80!black] at (9.38,0.970) {23};
\node[tlab, align=center, anchor=north] at (8.95,-0.08) {Identity \& Social\\group awareness};
\fill[red!22, draw=red!65!black, line width=0.5pt] (10.37,0) rectangle (10.77,0.434);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=red!65!black] at (10.57,0.442) {10};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (10.80,0) rectangle (11.20,0.312);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=blue!60!black] at (11.00,0.320) {7};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (11.23,0) rectangle (11.63,0.641);
\node[font=\fontsize{6.5}{7}\selectfont, anchor=south, text=orange!80!black] at (11.43,0.649) {15};
\node[tlab, align=center, anchor=north] at (11.00,-0.08) {Beyond-text\\features};
\fill[red!22, draw=red!65!black] (0.30,2.90) rectangle (0.54,3.05);
\node[font=\scriptsize, anchor=west] at (0.60,2.97) {rising};
\fill[blue!22, draw=blue!60!black] (4.27,2.90) rectangle (4.51,3.05);
\node[font=\scriptsize, anchor=west] at (4.57,2.97) {reaches its ceiling};
\fill[orange!30, draw=orange!80!black] (8.24,2.90) rectangle (8.48,3.05);
\node[font=\scriptsize, anchor=west] at (8.54,2.97) {bounded below 1};



==> figs/gen_osl_types8.tex <==
\draw[-{Stealth[length=1.6mm]}] (-0.25,0) -- (-0.25,2.80);
\node[tlab, rotate=90] at (-0.85,1.25) {share of regime (\%)};
\draw (-0.31,0.00) -- (-0.19,0.00); \node[tlab, anchor=east] at (-0.34,0.00) {0};
\draw (-0.31,0.50) -- (-0.19,0.50); \node[tlab, anchor=east] at (-0.34,0.50) {10};
\draw[black!12] (-0.19,0.50) -- (13.20,0.50);
\draw (-0.31,1.00) -- (-0.19,1.00); \node[tlab, anchor=east] at (-0.34,1.00) {20};
\draw[black!12] (-0.19,1.00) -- (13.20,1.00);
\draw (-0.31,1.50) -- (-0.19,1.50); \node[tlab, anchor=east] at (-0.34,1.50) {30};
\draw[black!12] (-0.19,1.50) -- (13.20,1.50);
\draw (-0.31,2.00) -- (-0.19,2.00); \node[tlab, anchor=east] at (-0.34,2.00) {40};
\draw[black!12] (-0.19,2.00) -- (13.20,2.00);
\draw (-0.31,2.50) -- (-0.19,2.50); \node[tlab, anchor=east] at (-0.34,2.50) {50};
\draw[black!12] (-0.19,2.50) -- (13.20,2.50);
\draw (-0.25,0) -- (13.20,0);
\fill[red!22, draw=red!65!black, line width=0.5pt] (0.12,0) rectangle (0.52,0.543);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (0.32,0.551) {11};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (0.55,0) rectangle (0.95,0.514);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (0.75,0.522) {10};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (0.98,0) rectangle (1.38,0.231);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (1.18,0.239) {5};
\node[tlab, align=center, anchor=north] at (0.82,-0.08) {surface \&\\compliance};
\fill[red!22, draw=red!65!black, line width=0.5pt] (1.77,0) rectangle (2.17,0.837);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (1.97,0.845) {17};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (2.20,0) rectangle (2.60,1.713);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (2.40,1.721) {34};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (2.63,0) rectangle (3.03,0.692);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (2.83,0.700) {14};
\node[tlab, align=center, anchor=north] at (2.47,-0.08) {local patterns\\(punchline, endings)};
\fill[red!22, draw=red!65!black, line width=0.5pt] (3.42,0) rectangle (3.82,1.386);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (3.62,1.394) {28};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (3.85,0) rectangle (4.25,0.935);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (4.05,0.943) {19};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (4.28,0) rectangle (4.68,1.154);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (4.48,1.162) {23};
\node[tlab, align=center, anchor=north] at (4.12,-0.08) {extended\\structure};
\fill[red!22, draw=red!65!black, line width=0.5pt] (5.07,0) rectangle (5.47,0.922);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (5.27,0.930) {18};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (5.50,0) rectangle (5.90,0.639);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (5.70,0.647) {13};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (5.93,0) rectangle (6.33,0.462);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (6.13,0.470) {9};
\node[tlab, align=center, anchor=north] at (5.77,-0.08) {evidence\\\& rigor};
\fill[red!22, draw=red!65!black, line width=0.5pt] (6.72,0) rectangle (7.12,0.192);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (6.92,0.200) {4};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (7.15,0) rectangle (7.55,0.156);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (7.35,0.164) {3};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (7.58,0) rectangle (7.98,0.308);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (7.78,0.316) {6};
\node[tlab, align=center, anchor=north] at (7.42,-0.08) {originality};
\fill[red!22, draw=red!65!black, line width=0.5pt] (8.37,0) rectangle (8.77,0.362);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (8.57,0.370) {7};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (8.80,0) rectangle (9.20,0.265);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (9.00,0.273) {5};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (9.23,0) rectangle (9.63,0.231);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (9.43,0.239) {5};
\node[tlab, align=center, anchor=north] at (9.07,-0.08) {audience\\fit};
\fill[red!22, draw=red!65!black, line width=0.5pt] (10.02,0) rectangle (10.42,0.238);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (10.22,0.246) {5};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (10.45,0) rectangle (10.85,0.405);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (10.65,0.413) {8};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (10.88,0) rectangle (11.28,1.154);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (11.08,1.162) {23};
\node[tlab, align=center, anchor=north] at (10.72,-0.08) {community \&\\identity};
\fill[red!22, draw=red!65!black, line width=0.5pt] (11.67,0) rectangle (12.07,0.520);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=red!65!black] at (11.87,0.528) {10};
\fill[blue!22, draw=blue!60!black, line width=0.5pt] (12.10,0) rectangle (12.50,0.374);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=blue!60!black] at (12.30,0.382) {7};
\fill[orange!30, draw=orange!80!black, line width=0.5pt] (12.53,0) rectangle (12.93,0.769);
\node[font=\fontsize{4.5}{5}\selectfont, anchor=south, text=orange!80!black] at (12.73,0.777) {15};
\node[tlab, align=center, anchor=north] at (12.37,-0.08) {beyond-text\\outcomes};
\fill[red!22, draw=red!65!black] (0.30,2.90) rectangle (0.54,3.05);
\node[font=\tiny, anchor=west] at (0.60,2.97) {rising};
\fill[blue!22, draw=blue!60!black] (4.56,2.90) rectangle (4.80,3.05);
\node[font=\tiny, anchor=west] at (4.86,2.97) {reaches its ceiling};
\fill[orange!30, draw=orange!80!black] (8.82,2.90) rectangle (9.06,3.05);
\node[font=\tiny, anchor=west] at (9.12,2.97) {bounded below 1};



==> figs/gen_tacit_iso.tex <==
\node[font=\scriptsize\bfseries, anchor=west] at (0.0,4.18) {the same criterion (\textsc{humor} bank: ``verbal economy and clarity''), decompressed for three executor scales};
\draw[black!40, fill=black!4, rounded corners=3pt] (0.00,0.12) rectangle (4.30,3.92);
\node[font=\scriptsize\bfseries, anchor=north west, align=left] at (0.10,3.86) {(1) \textsc{name}};
\node[draw=black!60, fill=white, rounded corners=1.5pt, font=\tiny, inner sep=3pt, align=left] (msg0) at (2.15,2.46) {Verbal economy and clarity};
\node[draw=violet!60!black, fill=violet!8, rounded corners=4pt, font=\small, align=center, inner sep=4pt] (exe0) at (2.15,1.30) {Llama-70B};
\draw[-{Stealth[length=1.8mm]}, thick] (msg0.south) -- (exe0.north);
\node[draw=black!60, fill=white, rounded corners=2pt, font=\tiny, inner sep=2.5pt] (bits0) at (2.15,0.52) {Reconstruction: \textbf{.049 bits}};
\draw[-{Stealth[length=1.6mm]}, thick] (exe0.south) -- (bits0.north);
\node[font=\Large\bfseries, text=black!70] at (4.51,2.00) {$\approx$};
\draw[black!40, fill=black!4, rounded corners=3pt] (4.72,0.12) rectangle (9.02,3.92);
\node[font=\scriptsize\bfseries, anchor=north west, align=left] at (4.82,3.86) {(2) \textsc{Name + Definition}};
\node[draw=black!60, fill=white, rounded corners=1.5pt, font=\tiny, inner sep=3pt, align=left] (msg1) at (6.87,2.46) {Verbal Economy and Clarity: A \\ text satisfies this criterion if every \\ word is essential to its \\ intended meaning and rhythm.};
\node[draw=blue!60!black, fill=blue!8, rounded corners=4pt, font=\small, align=center, inner sep=4pt] (exe1) at (6.87,1.30) {Llama-8B};
\draw[-{Stealth[length=1.8mm]}, thick] (msg1.south) -- (exe1.north);
\node[draw=black!60, fill=white, rounded corners=2pt, font=\tiny, inner sep=2.5pt] (bits1) at (6.87,0.52) {\textbf{.050 bits}};
\draw[-{Stealth[length=1.6mm]}, thick] (exe1.south) -- (bits1.north);
\node[font=\Large\bfseries, text=black!70] at (9.23,2.00) {$\approx$};
\draw[black!40, fill=black!4, rounded corners=3pt] (9.44,0.12) rectangle (13.74,3.92);
\node[font=\scriptsize\bfseries, anchor=north west, align=center] at (9.54,3.86) {(3) \textsc{Name +} \textsc{Definition +} \\ \textsc{Explanation}};
\node[draw=black!60, fill=white, rounded corners=1.5pt, font=\tiny, inner sep=3pt, align=left] (msg2) at (11.59,2.46) {Verbal Economy and Clarity: A text \\ satisfies this criterion if... in addition, \\ use: concise sentence structure, clear \\ narrative flow, no filler words... --- each word \\ contributes to the humorous effect because...};
\node[draw=green!45!black, fill=green!9, rounded corners=4pt, font=\small, align=center, inner sep=4pt] (exe2) at (11.59,1.30) {Llama-3B};
\draw[-{Stealth[length=1.8mm]}, thick] (msg2.south) -- (exe2.north);
\node[draw=black!60, fill=white, rounded corners=2pt, font=\tiny, inner sep=2.5pt] (bits2) at (11.59,0.52) {\textbf{.048 bits}};
\draw[-{Stealth[length=1.6mm]}, thick] (exe2.south) -- (bits2.north);



==> figs/gen_unit_decomp.tex <==
\node[lab, anchor=west, font=\small\bfseries\upshape] at (0.00,9.20) {A.\ \ Where units come from};
\node[draw=blue!60!black, fill=blue!12, rounded corners=2pt, text width=13.5mm, align=center, font=\Tiny, inner sep=2.5pt] (srcw) at (0.60,7.62) {\textbf{$s_1$: Mining explicit metrics online}\\[2pt] \tikz{\draw[black!55] (0,0) circle (0.16); \draw[black!45] (-0.16,0) arc (180:360:0.16 and 0.06); \draw[black!45] (0,-0.16) arc (270:90:0.06 and 0.16);}};
\node[draw=green!50!black, fill=green!12, rounded corners=2pt, text width=25mm, align=center, font=\Tiny, inner sep=3pt] (seed) at (2.60,7.80) {\textbf{$s_2$: Mining from GEPA trajectories}\\[1.5pt] \tikz{\node[draw=black!40, fill=white, rounded corners=1.5pt, text width=22mm, align=left, font=\Tiny, inner sep=2.5pt] {``Read the retrieved passages and \colorbox{green!25}{write a concise summary} of what they say about the question; issue a \colorbox{cyan!22}{follow-up search query} for what is missing; then answer.''};}\\[0.5pt] {\itshape the GEPA-optimized prompt $p_{\mathrm{gepa}}$}};
\node[draw=violet!60!black, fill=violet!12, rounded corners=2pt, text width=14.5mm, align=center, font=\Tiny, inner sep=2.5pt] (prop) at (4.88,7.62) {\textbf{$s_3$: Proposing from LLM}\\[1pt] \tikz{\foreach \i in {0,1,2}{\fill[blue!45!black] (0,\i*0.14) circle (0.035);} \foreach \i in {0,1}{\fill[blue!45!black] (0.30,0.07+\i*0.14) circle (0.035);} \fill[blue!45!black] (0.60,0.14) circle (0.035); \foreach \i in {0,1,2}{\foreach \j in {0,1}{\draw[blue!35, line width=0.3pt] (0.035,\i*0.14) -- (0.265,0.07+\j*0.14);}} \foreach \j in {0,1}{\draw[blue!35, line width=0.3pt] (0.335,0.07+\j*0.14) -- (0.565,0.14);}}\\[1pt] \textit{``propose clauses determining concise summaries''}};
\node[draw=black!22, fill=white, rounded corners=1.5pt, minimum width=30mm, minimum height=5mm] at (3.15,5.95) {};
\node[draw=black!25, fill=white, rounded corners=1.5pt, minimum width=30mm, minimum height=5mm, font=\tiny, text=black!40] at (2.85,6.08) {\ldots 68 candidates \ldots};
\node[draw=green!50!black, fill=green!14, rounded corners=1.5pt, font=\Tiny, text width=2.25cm, align=left, inner sep=2.5pt] (uok) at (1.58,5.74) {$u_{7}$: ``short, exact entity name or phrase, no filler\ldots''};
\node[draw=red!60!black, fill=red!10, rounded corners=1.5pt, font=\Tiny, text width=2.25cm, align=left, inner sep=2.5pt] (ubad) at (4.12,5.74) {$u_{44}$: ``synthesize summary\_1 and summary\_2\ldots''};
\draw[darr] (srcw.south) -- (1.80,6.25);
\draw[darr] (seed.south) -- (2.85,6.32);
\draw[darr] (prop.south) -- (3.90,6.25);
\node[blk, text width=1.9cm, font=\scriptsize\bfseries, draw=blue!50!black, fill=blue!6] (audit) at (2.85,3.30) {Audit};
\draw[arr, green!50!black] (uok.south) .. controls +(0.3,-0.5) .. (audit.north west);
\draw[arr, red!60!black] (ubad.south) .. controls +(-0.3,-0.5) .. (audit.north east);
\node[draw=red!60!black, fill=red!8, rounded corners=2pt, font=\scriptsize, inner sep=3.5pt, align=center] (disc) at (0.98,2.30) {\textcolor{red!60!black}{\textbf{$\times$}} reject (41)};
\draw[arr, red!60!black] (audit.south) .. controls +(-0.55,-0.4) .. (disc.east) node[pos=0.75, below=2pt, lab, red!60!black] {$\Delta\!\approx\!0$};
\draw[fill=black!6, draw=black!35, line width=0.8pt] plot[smooth cycle, tension=0.78] coordinates {(6.7,7.15) (8.7,7.9) (10.9,7.6) (11.85,6.0) (11.6,3.6) (10.1,2.5) (7.7,2.45) (6.35,3.9) (6.2,5.7)};
\draw[densely dashed, black!30] plot[smooth cycle, tension=0.78] coordinates {(6.35,7.55) (8.7,8.35) (11.25,8.0) (12.35,6.0) (12.05,3.3) (10.3,2.0) (7.55,1.95) (5.95,3.65) (5.8,5.8)};
\node[lab, black!45, anchor=west] at (10.90,2.05) {$\widehat N$: unmined};
\node[lab, anchor=west, font=\scriptsize\bfseries\upshape] at (6.85,7.40) {pool $\Omega$: 27 kept (11 shown)};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (6.90,6.78) {exact entity or date only\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (8.90,6.92) {person$\to$name; year$\to$4 digits\ldots};
\node[unit, fill=green!28, draw=green!50!black, line width=1.1pt, font=\tiny, inner sep=2pt, anchor=west, name=chipH] at (7.30,6.16) {short, exact entity phrase\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (9.10,6.30) {strictly concise format\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (6.75,5.54) {re-read the constraint list\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (9.00,5.66) {no filler, no reasoning\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (7.20,4.92) {link entities across summaries\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (9.12,5.02) {answer matches question type\ldots};
\node[unit, fill=cyan!20, draw=cyan!60!black, line width=1.1pt, font=\tiny, inner sep=2pt, anchor=west] at (6.90,4.30) {highly specific search query\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (9.05,4.38) {propose, then critique\ldots};
\node[unit, fill=green!12, draw=green!45!black, line width=0.5pt, font=\tiny, inner sep=2pt, anchor=west] at (8.05,3.62) {use only the summaries\ldots};
\draw[arr, green!50!black, line width=1.1pt] (audit.south) .. controls +(0.5,-1.0) and +(-2.2,-0.2) .. (chipH.west) node[pos=0.60, above=2pt, lab, green!45!black] {into $\Omega$ (27)};
\node[lab, anchor=west, font=\small\bfseries\upshape] at (12.55,9.20) {B.\ \ Inside the audit};
\draw[draw=blue!50!black, fill=blue!3, rounded corners=6pt, line width=1.0pt] (12.55,0.80) rectangle (16.62,8.25);
\node[anchor=north, font=\scriptsize\bfseries, text=blue!50!black, fill=blue!8, rounded corners=2pt, inner sep=2.5pt] at (14.58,8.18) {Audit};
\node[blk, text width=3.35cm, font=\scriptsize, draw=blue!50!black] (b1) at (14.58,7.28) {\textbf{1\ standalone screen}\\ \textcolor{black!55}{\tiny paired marginal vs.\ $p_{\mathrm{gepa}}$: $\Delta>0$, strict (1 pass)}};
\node[blk, text width=3.35cm, font=\scriptsize, draw=blue!50!black] (b2) at (14.58,6.19) {\textbf{2\ conditional gate}\\ \textcolor{black!55}{\tiny $\Delta(\Omega\oplus u \mid \Omega)>0$, strict ($\varepsilon{=}0$)}};
\draw[arr] (b1.south) -- (b2.north);
\node[blk, text width=3.35cm, font=\scriptsize, draw=black!45] (b3) at (14.58,5.10) {\textbf{3\ paired $k$-pass rescore}\\ \textcolor{black!55}{\tiny $k{=}5$ passes, same items, same session}};
\draw[arr] (b2.south) -- (b3.north);
\node[blk, text width=3.35cm, font=\scriptsize, draw=black!45] (b4) at (14.58,4.01) {\textbf{4\ shuffled control}\\ \textcolor{black!55}{\tiny scrambled $u$: expect $\Delta{\approx}0$ (no gate)}};
\draw[arr] (b3.south) -- (b4.north);
\node[blk, text width=3.35cm, font=\scriptsize, draw=black!45] (b5) at (14.58,2.92) {\textbf{5\ foreign control}\\ \textcolor{black!55}{\tiny other task's units: expect $\Delta{\approx}0$ (no gate)}};
\draw[arr] (b4.south) -- (b5.north);
\node[blk, text width=3.35cm, font=\scriptsize, draw=black!45] (b6) at (14.58,1.83) {\textbf{6\ removal probe}\\ \textcolor{black!55}{\tiny drop $u$ iff removal costs nothing ($\Delta_{\mathrm{drop}}\ge 0$)}};
\draw[arr] (b5.south) -- (b6.north);
\draw[decorate, decoration={brace, amplitude=4pt}, black!55] (16.80,7.62) -- (16.80,5.50) node[midway, right=4pt, lab, black!55, align=left] {per-unit\\ gates};
\draw[decorate, decoration={brace, amplitude=4pt}, black!55] (16.80,5.30) -- (16.80,1.05) node[midway, right=4pt, lab, black!55, align=left] {pool-level\\ audits\\ (post-hoc)};


